A First-Order Logic with Frames

We propose a novel logic, called Frame Logic (FL), that extends first-order logic (with recursive definitions) using a construct Sp(.) that captures the implicit supports of formulas -- the precise subset of the universe upon which their meaning depends. Using such supports, we formulate proof rules that facilitate frame reasoning elegantly when the underlying model undergoes change. We show that the logic is expressive by capturing several data-structures and also exhibit a translation from a precise fragment of separation logic to frame logic. Finally, we design a program logic based on frame logic for reasoning with programs that dynamically update heaps that facilitates local specifications and frame reasoning. This program logic consists of both localized proof rules as well as rules that derive the weakest tightest preconditions in FL.

==> frames.tex <==
% file not used anymore, has been integrated into frame-logic.tex
\section{Inductive Definitions and Frames}\label{sec:frames}


The relation symbols $I \in \I$ represent inductively defined
relations. Formally, an inductive definition is of the form
\[
\varphi_I =
\forall \overline{x}:\overline{\tau}. I(\overline{x}) \lfpiff
\rho_I(\overline{x})
\]
In the intended meaning, $I$ is interpreted as the least fixpoint that
satisfies this equation.  The usual requirement for inductive
definitions to be well defined is that the definition of $I$ does not
negatively depend on $I$. Recall that we have forbidden the use of inductive
predicates in guards of $\ite$-formulas and guards of existential
formulas. Further, we require that in
$\rho_I(\overline{x})$ each occurrence of an inductive predicate $I'$
is either inside a term $H(\varphi)$, or it occurs under an even
number of negations.\footnote{As usual, it would be sufficient to
  forbid negative occurrences of inductive predicates in mutual
  recursion.}   Below, we illustrate why we do not forbid negative
occurrences of inductive predicates inside terms $H(\varphi)$, in general.
%\todo[inline]{Maybe the last sentence is not necessary.}

We have not yet defined the intended semantics of the
terms $H(\varphi)$. For the moment, think of $H(\varphi)$ as the set
of elements on which mutable functions are dereferenced in order to
check the truth value of $\varphi$.

Consider the inductive definition of a predicate
$\mathit{tree}(x)$ w.r.t.\ two unary mutable functions $\ell$ and $r$:
\[
\begin{array}{ll}
  \mathit{tree}(x) &\lfpiff \ite(x = \nil: \top,\\
  &\mathit{tree}(\ell(x)) \land \mathit{tree}(r(x)) \land \\
  &H(\mathit{tree}(\ell(x))) \cap H(\mathit{tree}(r(x))) = \emptyset)
\end{array}
\]
In order to check whether the predicate $\mathit{tree}$ holds at some
element $u$, one needs to go down the pointers $\ell$ and $r$ starting
from $u$ until reaching $\nil$. Correspondingly, the heaplet
$\sem{H(\mathit{tree}(x))}(u)$ of the predicate
$\mathit{tree}$ at the element $u$ then consists of all these elements
that are encountered when following the pointers $\ell$ and $r$
starting from $u$. The requirement $H(\mathit{tree}(\ell(x))) \cap
H(\mathit{tree}(r(x))) = \emptyset$ corresponds to the property
of a tree that the left and right subtree are disjoint.

The formula $H(\mathit{tree}(\ell(x))) \cap H(\mathit{tree}(r(x))) =
\emptyset$ is a negative reference to the heaplets
$H(\mathit{tree}(\ell(x)))$ and $H(\mathit{tree}(r(x)))$ because the
emptiness of the intersection means that there does \emph{not} exist
an element that is contained in both heaplets.  This explains why we need
negative references to the heaplet of an inductively defined relation
$I$ inside the definition of $I$ (if we want to obtain a logic that
can define data structures like trees).

Since the heaplets are themselves defined inductively, we need to
ensure that the definition of the heaplet of $I$ does not depend on
$I$, otherwise the existence of the least fixpoint for the heaplets
and the inductive definitions would not be guaranteed.  The recursive
equations for the heaplet definitions given further below are such
that the heaplet of of formula is mainly defined via the syntax of the
formula, and not its semantics. The only exception are the guards in
$\ite$-formulas and existential formulas. For this reason, we have
required in the definition of formulas that guards do not contain
inductive relation symbols. This ensures that heaplets are independent
of the semantics of the inductive relations.


In the heaplet semantics, we are interested in models in which each $I
\in \I$ is the least fixpoint of its definition, and furthermore, the
heaplets $\sem{H(\varphi)}$ are interpreted as specific sets.

Formally, we define a family of equations, and require that the
interpretations $\sem{I}$ for each $I \in \I$ and the interpretations
$\sem{H(\varphi)}$ correspond to the the simultaneous least fixpoint
of these equations.

\begin{definition}\label{def:heaplet-equations}
Let $M$ be a model as defined in Section~\ref{sec:frame-logic}

\begin{itemize}
\item The equations for the inductive definitions are:
\[
\sem{I} = \sem{\rho_I}
\]
\item The equations for the heaplets of terms are
  \[
  \begin{array}{rcl}
    \sem{H(c)}(\nu) &=& \emptyset \mbox{ for a constant $c$}\\
    \sem{H(x)}(\nu) &=& \emptyset \mbox{ for a variable $x$}\\
  \sem{H(f(t_1, \ldots, t_n))}(\nu) &=&
  \begin{cases}
  \bigcup\limits_{i \text{ with } t_i \text{ of sort } \fs}\{\semnu{t_i}\} \cup \bigcup\limits_{i=1}^n \sem{H(t_i)}(\nu) & \mbox{if } f \in \Fm \\
  \bigcup\limits_{i=1}^n \sem{H(t_i)}(\nu) & \mbox{if } f \not\in \Fm 
  \end{cases}\\
  \sem{H(H(\varphi))}(\nu) &=& \sem{H(\varphi)}(\nu)
    \end{array}
  \]
\item The equations for the heaplets of formulas are
  \[
  \begin{array}{rcl}
\sem{H(R(t_1, \ldots, t_n))}(\nu) &=& \bigcup_{i=1}^n \sem{H(t_i)}(\nu)  \mbox{
  for $R \in \R$}\\
 \sem{H(t_1 = t_2)}(\nu) &=& \sem{H(t_1)}(\nu) \cup \sem{H(t_2)}(\nu) \\
\sem{H(I(t_1, \ldots, t_n)}(\nu) &=& \sem{H(\rho_I(t_1,\ldots,t_n))}(\nu) \cup \bigcup_{i=1}^n \sem{H(t_i)}(\nu)  \mbox{
  for $I \in \I$} \\
\sem{H(\varphi_1 \land \varphi_2)}(\nu) &=& \sem{H(\varphi_1)}(\nu) \cup
\sem{H(\varphi_2)}(\nu) \\
\sem{H(\lnot \varphi)}(\nu) &=& \sem{H(\varphi)}(\nu) \\
\sem{H(\ite(\gamma:\varphi_1,\varphi_2))}(\nu)  &=& \sem{H(\gamma)}(\nu) \cup
  \begin{cases}
     \sem{H(\varphi_1)}(\nu) \mbox{ if } M \models \gamma \\
    \sem{H(\varphi_2)}(\nu) \mbox{ if } M \not\models \gamma 
  \end{cases} \\
\sem{H(\ite(\gamma:t_1,t_2))}(\nu)  &=& \sem{H(\gamma)}(\nu) \cup
  \begin{cases}
     \sem{H(t_1)}(\nu) \mbox{ if } M \models \gamma \\
    \sem{H(t_2)}(\nu) \mbox{ if } M \not\models \gamma 
  \end{cases} \\
   \sem{H(\exists y: \gamma.\varphi)}(\nu) &=& \bigcup\limits_{u \in D_y} \sem{H(\gamma)}(\nu[y \leftarrow u]) \cup \bigcup\limits_{u \in D_y; M,\nu[y
      \leftarrow u] \models \gamma} \sem{H(\varphi)}(\nu[y \leftarrow u])
  \end{array}
  \]
\end{itemize}
\end{definition}

We are interested in models in which the interpretation of the
inductive relations and the heaplets corresponds to the 
least fixpoint of the above equations. The definitions are made such
that the least fixpoint for the heaplet expressions is independent of
the interpretation of the inductive relations, they only depend on the
syntactic definition of the inductive relations. This ensures that there
indeed exists a unique simultaneous least fixpoint of the equations for
the inductive relations and the heaplet expressions.
We refer to such models as \emph{heaplet models}. See Appendix~\ref{sec:heaplet-models} for rigorous formulation of heaplet models.

% \todo[inline]{The following formalization of heaplet models can go to the appendix.}

% \todo[inline]{End of part that can go to the appendix.}

The heaplet of a formula can be used for frame reasoning. If we modify
a model $M$ by changing the interpretation of the mutable functions
(e.g., a program modifying pointers), then the truth value of a
formula does not change if the change happens outside the heaplet of
the formula. This is formalized below.



Given two models $M,M'$ over the same universe, we say that $M'$ is a
\emph{mutation of $M$} if $\sem{R} = \sem[M']{R}$, $\sem{c} = \sem[M']{c}$, and $\sem{f} = \sem[M']{f}$,
for all constants $c$, relations $R \in \R$, and
functions $f \in F \setminus \Fm$. In other words, the pre-model of
$M$ only differs from the pre-model of $M'$ on the interpretations of
the mutable functions.

Given a subset $X \subseteq U_{\sf}$ of the elements from the
foreground universe, we say that the \emph{mutation is stable on $X$}
if the values of the mutable functions did not change on arguments
from $X$. More formally, if for all mutable functions $f \in \Fm$ and
all appropriate tuples $u_1, \ldots, u_n$ of arguments, $\{u_1, \ldots,
u_n\} \cap X \not= \emptyset$ implies $\sem{f}(u_1, \ldots, u_n) =
\sem[M']{f}(u_1, \ldots, u_n)$.

\begin{theorem}[Frame Theorem] 
Let $M,M'$ be heaplet models such that $M'$ is a mutation of $M$ that is
stable on $X \subseteq U_{\fs}$. Let $\nu$ be a variable assignment
and $\varphi$ be a formula
with $\sem{H(\varphi)}(\nu) \subseteq X$.
Then $M,\nu \models \varphi$ iff $M',\nu \models \varphi$.
\end{theorem}
\todo[inline]{Proof should go to the appendix because it uses the formal definitions of the heaplet models.}
\begin{proof}
See Appendix~\ref{sec:omitted-proofs}.
\end{proof}



==> intuition.tex <==
% file not used anymore, has been integrated into frame-logic.tex
\section{Intuition behind frame semantics}

\todo[inline]{Madhu: Writing regarding design decisions for heaplets; should be merged into the formal definitions.}

We now discuss the design decisions that go behind the semantics of the frame operator $Fr$ in our logic. The first decision, as described in the introduction, is to have every formula define uniquely a frame, which roughly captures the subdomain of mutable functions that a formula
$\varphi$'s truthhood depends on, 
and have $\Fr(\varphi)$ evaluate to it.

The choice for frames of atomic formulae are relatively clear. An atomic formula of the kind
$f(x)=y$, where $x$ is of the foreground sort and $f$ is a mutable function, has as its frame the singleton set containing the location $x$. And atomic formulas that do not involve mutable functions over the foreground have an empty frame. Frames for terms can also be similarly defined. The frame of a conjunction $\alpha \wedge \beta$ should clearly be the union of the frames of the two formulas.

What should the frame of a formula $\alpha \vee \beta$ be? The choice we make here is that its frame is the \emph{union} of the frames of $\alpha$ and $\beta$. Note that in a model where $\alpha$ is true and $\beta$ is false, we still include the heaplet of $\beta$ in $\Fr(\alpha \vee \beta)$. In a sense, this is an overapproximation of the frame as far as frame reasoning goes, as surely preserving the model's definitions on the frame of $\alpha$ will preserve 
the truth of $\alpha$. 

However, we prefer the frame to be the union of the frames of $\alpha$ and $\beta$. We think of the frame as the subdomain of the universe that determines the meaning of the formula, whether it be \emph{true} or \emph{false}. Consequently, we would like
the frame of a formula and its negation to be the
same. Given that the frame of the negation of a disjunction, being a conjunction, would be the union of the frames of $\alpha$ and $\beta$, we would like this to be the frame. 

Separation logic makes a different design decision.
Logical formulas are not associated with tight frames, but rather, the semantics of the formula is defined for models with given frames/heaplets, 
where the idea of a heaplet is whether it supports
the \emph{truthhood} of a formula (and not its falsehood).
For example, for a model, the various heaplets that satisfy $\neg (f(x)=y)$ in separation logic would include all heaplets where the location of $x$ is not present, which does not coincide with the notion we have for frames.
However, for positive formulas, separation logic handles frames more accurately, as it can associate several frames for a formula. For example, the heaplets for $\alpha \vee \beta$, when both $\alpha$ and $\beta$ are true in a model, would include two heaplets, one being the heaplet of $\alpha$, and the other being the heaplet of $\beta$. Note that a change
to the model that does not affect one of these heaplets does ensure the formula continues to hold true, and can be argued by frame reasoning. 
The decision to have a single frame for a formula compels us to take the union of the frames to be the frame of a disjunction.

There are situations, however, where there are disjunctions $\alpha \vee \beta$, where only \emph{one} of the disjuncts can possibly be true, and hence we would like the frame of the formula to be the frame of the disjunct that happens to be true. An example of this is when $\alpha$ is of the form $p \wedge \alpha'$ and $\beta$ is of the form $\neg p \wedge \beta'$, where, say, $p$ is a formula with an empty frame. In this case, we would like the frame of the disjunction to be the frame of $\alpha$, if $p$ is true, and the frame of $\beta$, if $p$ is false. 

We therefore introduce a new syntactical form $ite(\gamma: \alpha, \beta)$ in frame logic, whose heaplet is the union of the frames of $\gamma$ and $\alpha$, if $\gamma$ is true, and the frames of $\gamma$ and $\beta$ if $\gamma$ is false. While the truthhood of 
$ite(\gamma: \alpha, \beta)$ is the same as
that of $(\gamma \wedge \alpha) \vee (\neg \gamma \wedge \beta)$, its frames are potentially smaller,
allowing us to write formulas with tighter frames
to support better frame reasoning. Note that the
frame of $ite(\gamma, \alpha, \beta)$ and its negation $ite(\gamma, \neg \alpha, \neg \beta)$ are the same, as we desired.

Turning to quantification, the frame for a formula of the form $\exists x. \alpha$ is hard to define, as its truthhood could depend on the entire universe.
We hence provide a mechanism for \emph{guarded}
quantification, in the form $\exists x: \gamma. ~~\alpha$. The semantics of this formula is
that there exists some location that satisfies the guard $\gamma$, for which $\alpha$ holds. 
The frame for such a formula includes
the frame of the guard, and the frames of $\alpha$
when $x$ is interpreted to be a location that satisfies $\gamma$. For example, $\exists x: (x=f(y)).~~g(x)=z$ has as its frame the locations interpreted for $y$ and $f(y)$ only.

There are several technicalities in defining the semantics, especially in giving least fixpoint semantics to recursive definitions which themselves can involve frame expressions.
The resolution of these difficulties forces us to impose certain restrictions on the syntax of the logic. For instance, we disallow guards in $ite$ and existentially quantified expressions to contain
recursively defined relations.

\todo{Add more restrictions}

